MemRetriever: Learning to Search, Reflect, and Retrieve from Long-Term Memory

Long-term memory enables personalized agents, but its value depends on retrieving the right evidence at the right time. Most memory systems use static top-k retrieval: they issue one query, return a fixed number of memories, and pass them directly to a downstream model. This approach can miss evidence distributed across sessions, introduce irrelevant content, and waste context, especially for multi-hop, temporal, and knowledge-update questions. We present MemRetriever, an agentic retrieval model that treats memory access as a multi-step search process. At each step, MemRetriever reasons over the current evidence and selects parallel search for broad exploration, serial search for targeted completion, or reflection and denoising for filtering and evidence assessment. It stops when the retained evidence is sufficient for downstream answering. We construct ReAct-style search-memory trajectories for supervised warm-start training and further optimize the model with Group Relative Policy Optimization. The reward design encourages evidence coverage, noise reduction, answer sufficiency, and efficient termination. Experiments on LOCOMO, LongMemEval, HotpotQA, MuSiQue, and 2WikiMultiHopQA show consistent improvements over static retrieval and supervised-only baselines. MemRetriever-4B-RL also outperforms DeepSeek-v4-Flash on the main LongMemEval retrieval metrics under the same pipeline and achieves the strongest results among the compared methods on MuSiQue. Because its decision logic is independent of the storage backend, MemRetriever can also operate over external knowledge bases and vector databases. These results show that an intermediate decision layer that plans, searches, filters evidence, and determines when to stop can improve both long-term memory retrieval and knowledge-intensive question answering.

==> prism-uploads/case_study_latex.tex <==
% ============================================================
% 在 preamble 中加入以下包和样式定义
% ============================================================
\usepackage{tcolorbox}
\usepackage{enumitem}
\usepackage{xcolor}
\usepackage{fontawesome5}  % 用于图标（可选）

\tcbuselibrary{skins, breakable}

% ---------- 颜色定义 ----------
\definecolor{qborder}{HTML}{378ADD}
\definecolor{qbg}{HTML}{E6F1FB}
\definecolor{thinkborder}{HTML}{AFA9EC}
\definecolor{thinkbg}{HTML}{F5F4FE}
\definecolor{retainedbg}{HTML}{EAF3DE}
\definecolor{retainedtext}{HTML}{27500A}
\definecolor{retainedborder}{HTML}{97C459}
\definecolor{discardedbg}{HTML}{F1EFE8}
\definecolor{discardedtext}{HTML}{888780}
\definecolor{answerbg}{HTML}{EAF3DE}
\definecolor{answerborder}{HTML}{639922}
\definecolor{serialbg}{HTML}{E6F1FB}
\definecolor{serialtext}{HTML}{0C447C}
\definecolor{parallelbg}{HTML}{E1F5EE}
\definecolor{paralleltext}{HTML}{085041}
\definecolor{reflectbg}{HTML}{FAECE7}
\definecolor{reflecttext}{HTML}{712B13}

% ---------- 样式定义 ----------
% 主 case 容器
\newtcolorbox{casebox}[1]{
  enhanced, breakable,
  colback=white, colframe=gray!30,
  fonttitle=\bfseries\small,
  title={#1},
  boxrule=0.4pt, arc=4pt,
  top=6pt, bottom=6pt, left=8pt, right=8pt,
  toptitle=4pt, bottomtitle=4pt,
}

% 问题框
\newtcolorbox{questionbox}{
  enhanced,
  colback=qbg, colframe=qborder,
  boxrule=0pt, leftrule=3pt, arc=0pt,
  top=4pt, bottom=4pt, left=8pt, right=8pt,
}

% Think 块
\newtcolorbox{thinkbox}{
  enhanced,
  colback=thinkbg, colframe=thinkborder,
  boxrule=0pt, leftrule=2pt, arc=0pt,
  top=3pt, bottom=3pt, left=6pt, right=6pt,
  fontupper=\small\itshape\color{gray!70!black},
}

% 答案框
\newtcolorbox{answerbox}{
  enhanced,
  colback=answerbg, colframe=answerborder,
  boxrule=0pt, leftrule=3pt, arc=0pt,
  top=4pt, bottom=4pt, left=8pt, right=8pt,
}

% ---------- 行内标签命令 ----------
\newcommand{\tagserial}{%
  \tikz[baseline=(tag.base)]{\node[fill=serialbg, text=serialtext,
    rounded corners=2pt, inner sep=2pt, font=\scriptsize\bfseries] (tag) {serial search};}%
}
\newcommand{\tagparallel}{%
  \tikz[baseline=(tag.base)]{\node[fill=parallelbg, text=paralleltext,
    rounded corners=2pt, inner sep=2pt, font=\scriptsize\bfseries] (tag) {parallel search};}%
}
\newcommand{\tagreflect}{%
  \tikz[baseline=(tag.base)]{\node[fill=reflectbg, text=reflecttext,
    rounded corners=2pt, inner sep=2pt, font=\scriptsize\bfseries] (tag) {reflect \& denoise};}%
}

% 证据条目命令
\newcommand{\evretained}[2]{%
  \par\noindent\colorbox{retainedbg}{%
    \parbox{\dimexpr\linewidth-2\fboxsep}{%
      \small\color{retainedtext}\textbf{[#1]}~#2%
    }%
  }\vspace{1pt}%
}
\newcommand{\evdiscarded}[2]{%
  \par\noindent\colorbox{discardedbg}{%
    \parbox{\dimexpr\linewidth-2\fboxsep}{%
      \small\color{discardedtext}\sout{[#1]~#2}%
    }%
  }\vspace{1pt}%
}

% 查询条目命令
\newcommand{\queryitem}[1]{%
  \par\noindent{\small\ttfamily\color{gray!70!black}#1}\vspace{1pt}%
}


% ============================================================
% 以下为正文中的使用示例
% ============================================================

\begin{figure*}[t]
\centering

% ==================== Case 1 ====================
\begin{casebox}{Case 1: Multi-hop knowledge retrieval \hfill \tikz[baseline=(tag.base)]{\node[fill=serialbg, text=serialtext, rounded corners=2pt, inner sep=2pt, font=\scriptsize\bfseries] (tag) {QA};}}

\begin{questionbox}
\textbf{Question:} The Russell Subdivision is a railroad line owned by a railroad headquartered in what state?
\end{questionbox}

\vspace{6pt}
\noindent\textbf{Step 1} \hfill \tagserial

\begin{thinkbox}
I first need to identify which railroad owns the Russell Subdivision. Once the owner is known, I can search for the headquarters location.
\end{thinkbox}

\noindent{\small\textbf{Query:} \texttt{Which railroad owns the Russell Subdivision?}}

\vspace{4pt}
\noindent{\scriptsize\textbf{Retrieved evidence:}}
\evretained{0}{The Russell Subdivision is a railroad line owned by CSX Transportation in the U.S. State of Kentucky.}
\evdiscarded{1}{The line runs from Russell, Kentucky to Greenup, Kentucky.}
\evdiscarded{2}{The Hudson Subdivision is a railroad line owned by CSX Transportation and leased by Amtrak in New York.}

\vspace{8pt}
\noindent\textbf{Step 2} \hfill \tagserial

\begin{thinkbox}
The first retrieval establishes CSX Transportation as the owner. The remaining missing information is the state where CSX is headquartered.
\end{thinkbox}

\noindent{\small\textbf{Query:} \texttt{Where is CSX Transportation headquartered?}}

\vspace{4pt}
\noindent{\scriptsize\textbf{Retrieved evidence:}}
\evretained{3}{CSX Transportation is headquartered in Jacksonville, Florida.}
\evdiscarded{4}{CSX Transportation is a Class I railroad in the United States.}
\evdiscarded{5}{CSX operates one of the three Class I railroads serving most of the East Coast.}

\vspace{8pt}
\noindent\textbf{Step 3} \hfill \tagreflect

\begin{thinkbox}
Evidence now supports the full chain: Russell Subdivision $\to$ CSX Transportation $\to$ Jacksonville, Florida. Retaining only the two key passages.
\end{thinkbox}

\noindent{\scriptsize\textbf{Final evidence pool:}}
\evretained{0}{Russell Subdivision is owned by CSX Transportation in Kentucky.}
\evretained{3}{CSX Transportation is headquartered in Jacksonville, Florida.}

\vspace{4pt}
\begin{answerbox}
{\scriptsize\textbf{Final answer (by working agent):}} \textbf{Florida.}
\end{answerbox}

\end{casebox}

\vspace{8pt}

% ==================== Case 2 ====================
\begin{casebox}{Case 2: Personal memory retrieval \hfill \tikz[baseline=(tag.base)]{\node[fill=parallelbg, text=paralleltext, rounded corners=2pt, inner sep=2pt, font=\scriptsize\bfseries] (tag) {Memory};}}

\begin{questionbox}
\textbf{Question:} What did Melanie realize after the charity race?
\end{questionbox}

\vspace{6pt}
\noindent\textbf{Step 1} \hfill \tagparallel

\begin{thinkbox}
The relevant memory may be phrased in different ways. I should issue several complementary searches around the race, what happened afterward, and Melanie's realization.
\end{thinkbox}

\noindent{\small\textbf{Queries:}}
\queryitem{q1: Melanie charity race realized after the race}
\queryitem{q2: charity race Melanie afterwards thought realized}
\queryitem{q3: Melanie race charity event conversation turned after race}

\vspace{4pt}
\noindent{\scriptsize\textbf{Retrieved evidence:}}
\evretained{0}{Melanie ran a charity race for mental health. She found it rewarding and reflected on the importance of mental health care.}
\evretained{1}{Melanie participated in a charity race for mental health. It prompted her to reflect on mental well-being and self-care.}
\evdiscarded{2}{Melanie participated in an advocacy event described as a cool experience with love and support.}
\evretained{3}{Caroline supported Melanie's participation and said raising awareness for mental health is rewarding.}

\vspace{8pt}
\noindent\textbf{Step 2} \hfill \tagreflect

\begin{thinkbox}
The pool contains direct evidence but also one noisy memory about a different advocacy event. Retaining memories about the charity race; discarding the unrelated event.
\end{thinkbox}

\noindent{\scriptsize\textbf{Final evidence pool:}}
\evretained{1}{Melanie participated in a charity race for mental health and reflected on mental well-being and self-care.}
\evretained{0}{Melanie found the charity race rewarding and reflected on the importance of mental health care.}
\evretained{3}{Caroline supported Melanie and emphasized that raising awareness for mental health is rewarding.}

\vspace{4pt}
\begin{answerbox}
{\scriptsize\textbf{Final answer (by working agent):}} \textbf{Melanie realized the importance of mental health care, mental well-being, and self-care.}
\end{answerbox}

\end{casebox}

\caption{Case study rollouts. \textbf{Case 1} demonstrates multi-hop knowledge retrieval via two serial searches followed by a reflect step. \textbf{Case 2} demonstrates personal memory retrieval via parallel search followed by a reflect step. Green entries denote retained evidence; struck-through gray entries denote discarded evidence.}
\label{fig:case-study}
\end{figure*}

